Egocentric Video-Language Pretraining @ Ego4D Challenge 2022

In this report, we propose a video-language pretraining (VLP) based solution \cite{kevin2022egovlp} for four Ego4D challenge tasks, including Natural Language Query (NLQ), Moment Query (MQ), Object State Change Classification (OSCC), and PNR Localization (PNR). Especially, we exploit the recently released Ego4D dataset \cite{grauman2021ego4d} to pioneer Egocentric VLP from pretraining dataset, pretraining objective, and development set. Based on the above three designs, we develop a pretrained video-language model that is able to transfer its egocentric video-text representation or video-only representation to several video downstream tasks. Our Egocentric VLP achieves 10.46R@1&IoU @0.3 on NLQ, 10.33 mAP on MQ, 74% Acc on OSCC, 0.67 sec error on PNR. The code is available at https://github.com/showlab/EgoVLP.

==> tex/mq_test.tex <==
\begin{table*}[htb]
\small
\centering
{
\begin{tabular}{clc|cc}
	\toprule
	\textbf{Methods} & \multicolumn{2}{c|}{\textbf{Video-text Pre-extrated Features}} & \multicolumn{1}{c}{\textbf{IoU=0.5}} & \multicolumn{1}{c}{\textbf{mAP$(\%)$IoU}} \\
	& Vis Enc & Vis-text PT & R@1  & Avg \\  \midrule[1pt] 
	VSGN &  SlowFast & - & $24.25$  & $5.68$   \\ \midrule
	VSGN & Frozen & \howto&  $18.06$  & $5.28$   \\
	VSGN & Frozen & CC3M+WebVid2M  & $19.74$  & $5.95$   \\
	VSGN & Frozen & \dataset  & \underline{$27.98$}  & \underline{$9.78$}   \\
	VSGN & Frozen+\model & \dataset & $\mathbf{28.03}$  & $\mathbf{10.33}$   \\
	\bottomrule
\end{tabular}
}
\centering
\caption{Recall and mAP metrics on the MQ task's test set.}
\label{mq_test}
\vspace{-1em}
\end{table*}

==> tex/nlq.tex <==
%\begin{wraptable}{rh}{0.6\textwidth}
\begin{table*}
\small
\centering
\vspace{-1.em}
\setlength{\tabcolsep}{3pt}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{clc|cccc}
	\toprule
	\textbf{Methods} & \multicolumn{2}{c|}{\textbf{Video-text Pre-extrated Features}} & \multicolumn{2}{c}{\textbf{IoU=0.3}} & \multicolumn{2}{c}{\textbf{IoU=0.5}} \\
	& Vis-text Enc & Vis-text PT & R@1 & R@5 & R@1 & R@5 \\  \midrule[1pt] 
	2D-TAN~\cite{zhang2020learning} &  SlowFast+BERT& - & $5.04$ & $12.89$ & $2.02$ & $5.88$   \\
	VSLNet~\cite{zhang2020span}  &  SlowFast+BERT   & - & $5.45$ & $10.74$ & $3.12$ & $6.63$  \\  
	 \midrule
 	VSLNet~\cite{zhang2020span}  &  Frozen       & \howto        & $3.95$ & $8.72$  & $2.01$ & $4.62$ \\	
	VSLNet~\cite{zhang2020span}  &  Frozen       & CC3M+WebVid2M & $5.06$ & $10.30$ & $2.71$ & $6.69$ \\		
	VSLNet~\cite{zhang2020span}  &  Frozen       & \dataset      & \underline{$10.53$} & \underline{$17.94$} & \underline{$5.96$} & \underline{$11.85$}\\
	VSLNet~\cite{zhang2020span}  &  Frozen+\model& \dataset      & $\mathbf{10.84}$ & $\mathbf{18.84}$ & $\mathbf{6.81}$ & $\mathbf{13.45}$ \\	
	\bottomrule
\end{tabular}
}
\centering
\caption{Recall for several IoU on the NLQ task's val. set.}
\vspace{-1em}
% \label{nlq}
%\end{wraptable}
\end{table*}

==> tex/nlq_test.tex <==
\begin{table*}[htb]
\small
\centering
\begin{tabular}{clc|cccc}
	\toprule
	\textbf{Methods} & \multicolumn{2}{c|}{\textbf{Video-text Pre-extrated Features}} & \multicolumn{2}{c}{\textbf{IoU=0.3}} & \multicolumn{2}{c}{\textbf{IoU=0.5}} \\
	& Vis-text Enc & Vis-text PT & R@1 & R@5 & R@1 & R@5 \\  \midrule[1pt] 
	VSLNet  &  SlowFast+BERT   & - & $5.47$ & $11.21$ & $2.80$ & $6.57$  \\  
	 \midrule
 	VSLNet  &  Frozen       & \howto        & $3.77$ & $6.87$  & $1.62$ & $3.45$ \\	
	VSLNet  &  Frozen       & CC3M+WebVid2M & $4.87$ & $8.67$ & $2.50$ & $4.97$ \\		
	VSLNet  &  Frozen       & \dataset      & \underline{$10.34$} & \underline{$15.81$} & \underline{$6.24$} & \underline{$10.39$}\\
	VSLNet  &  Frozen+\model& \dataset      & $\mathbf{10.46}$ & $\mathbf{16.76}$ & $\mathbf{6.24}$ & $\mathbf{11.29}$ \\	
	\bottomrule
\end{tabular}
\centering
\caption{Recall for several IoU on the NLQ task's test set.}
\label{nlq_test}
\vspace{-1em}
\end{table*}

==> tex/oscc.tex <==
\begin{wraptable}{rh}{0.45\textwidth}
\small
\centering
\vspace{-1.1em}
\setlength{\tabcolsep}{3pt}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lc|c}
	\toprule[1pt] 
	\textbf{Methods}  &  \textbf{Vis-Text PT} & \textbf{Acc.~(\%)} \\ \midrule[1pt] 
	Always Positive                          &  -        & $48.1$  \\
	Bi-d LSTM~\cite{graves2005bidirectional} &  ImageNet & $65.3$  \\
	I3D ResNet-50~\cite{carreira2017quo}     &  -        & $68.7$  \\ 
	\midrule
	Frozen &   -            & $70.3$              \\
	Frozen &  HowTo100M     & $71.7$              \\
	Frozen &  CC3M+WebVid2M & $71.5$              \\
	Frozen &  \dataset      & \underline{$73.4$}  \\
	Frozen+\model~ & \dataset  & $\mathbf{73.9}$ \\
	\bottomrule[1pt] 
\end{tabular}
}
\centering
\caption{Accuracy metric on the \ossc~ task's val set.}
\vspace{-2em}
\label{ossc}
\end{wraptable}

==> tex/pnr.tex <==
\begin{wraptable}{rh}{0.45\textwidth}
\small
\centering
\vspace{-1.1em}
\setlength{\tabcolsep}{3pt}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lc|c}
	\toprule[1pt] 
	\textbf{Methods}  &  \textbf{Vis-Text PT} & \textbf{Acc.~(\%)} \\ \midrule[1pt] 
	Always Positive                          &  -        & $48.1$  \\
	Bi-d LSTM~\cite{graves2005bidirectional} &  ImageNet & $65.3$  \\
	I3D ResNet-50~\cite{carreira2017quo}     &  -        & $68.7$  \\ 
	\midrule
	Frozen &   -            & $70.3$              \\
	Frozen &  HowTo100M     & $71.7$              \\
	Frozen &  CC3M+WebVid2M & $71.5$              \\
	Frozen &  \dataset      & \underline{$73.4$}  \\
	Frozen+\model~ & \dataset  & $\mathbf{73.9}$ \\
	\bottomrule[1pt] 
\end{tabular}
}
\centering
\caption{Accuracy metric on the \ossc~ task's val set.}
\vspace{-2em}
\label{ossc}
\end{wraptable}
